Asymptotic Purification of Quantum Trajectories under Random Generalized Measurements

We develop a general framework to study quantum trajectories resulting from repeated random measurements subject to stationary noise, and generalize results of K\"ummerer and Maassen to this setting. The resulting trajectory of quantum states is a time-inhomogeneous Markov chain in a random environment. K\"ummerer and Maassen introduced the concept of dark subspaces for noise-free processes, establishing that their absence is equivalent to asymptotic purification of the system state. We clarify the notion of dark subspaces in the disordered setting by defining a measurable correspondence consisting of a collection of random subspaces satisfying a darkness condition. We further prove that asymptotic purification occurs if and only if this collection of random dark subspaces is empty. Several examples of these phenomena are provided.

==> 4_proofs.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
We are now ready to provide proof of Theorem \ref{0-1 law for purification of disordered quantum trajectories}, which we restate below for the convenience of the reader.  
%
%
\firstresult*
%
%
\begin{proof}[Proof of Theorem \ref{0-1 law for purification of disordered quantum trajectories}]
First we note that from corollary \ref{Purification is an event} we have that $X$ is $\mcF$-measurable. Now we prove that $X$ is essentially $\theta$-invariant whence $\Pr(X) \in \{0,1\}$ follows from the ergodicity of $\theta$. To see that, we claim that for $\omega\in\Omega$, $\varrho\in\mbS_D$ and $a\in\mcA$ with $\tr{V_{a;\theta(\omega)} \varrho V_{a;\theta(\omega)}^\dagger} \neq 0$ we must have that for any $S\in\Sigma$
\begin{equation}
    \mbQ_{\varrho;\omega}\left(\{a\}\times S\right) = \tr{V_{a;\theta(\omega)}\varrho V_{a;\theta(\omega)}^\dagger} \times \mbQ_{\varrho'_{a;\omega};\theta(\omega)}\left(S\right)
\end{equation}
where
\begin{equation}
    \varrho'_{a;\omega} = V_{a;\theta(\omega)}\cdot \varrho = \dfrac{V_{a;\theta(\omega)} \varrho V_{a;\theta(\omega)}^\dagger}{\tr{V_{a;\theta(\omega)} \varrho V_{a;\theta(\omega)}^\dagger}}
\end{equation}

This can be established by, first observing that the statement holds for any $\{a_1\}\times\{a_2\}\ldots \{a_n\}\times\mcA\ldots $ where $(a_1,\ldots, a_n)$ is a finite sequence of points from $\mcA$. Thus the result holds for any $n$-level cylinder sets. Then the result extends to any $S\in\Sigma$ by a monotone class argument. Now let $\omega \in \theta^{-1}(X)$ then $\theta(\omega)\in X$ and thus by definition of $X$ we have that for any state $\varrho$, the quantum trajectory started at $\varrho$ with the disorder realization $\theta(\omega)$ purifies $\mbQ_{\varrho;\theta(\omega)}$-almost surely for all observed sequences of outcomes. In particular we must have that for any state $\varrho$ and $a\in\mcA$ whenever $ \varrho': = V_{a;\theta(\omega)}\cdot \varrho \in\mbS_D$ the quantum trajectory started at $\varrho'$ with disorder $\theta(\omega)$ purifies  $\mbQ_{\varrho';\theta(\omega)}$-almost surely for all observed sequences of outcomes. Thus there is some $B\in\Sigma$ with $\mbQ_{\varrho';\omega}(B) = 1$ and for any $\bar{a}\in B$ we have that $M^{(m,\infty)}_{\varrho';\theta(\omega)}(\bar(a)) = 1$. Thus by previous claim we have that for $B' = \cup_{a\in\mcA} \{a\}\times B$
    \begin{equation}
        \mbQ_{\varrho;\omega}(B') = \sum_{a\in\mcA} \mbQ_{\varrho;\omega}\left(\{a\} \times B\right) = \sum_{a\in\mcA} 
        \ \left[ \tr{V_{a;\theta(\omega)}\varrho V_{a;\theta(\omega)}^\dagger} \times \mbQ_{\varrho';\theta(\omega)}\left(B\right)\right] = 1
    \end{equation}
Furthermore for any $\bar{b}\in \cup_{a\in\mcA} \{a\} \times B$ such that $\bar{b} = (a,a_1,a_2\ldots )$ we have that 
\begin{align}
    \rho^{(n)}_{\varrho;\omega} (\bar{b}) &= \dfrac{ V_{a_n;\theta^{n+1}(\omega)} \ldots V_{a_1;\theta^2(\omega)} V_{a;\omega} \varrho V_{a;\omega}^\dagger V_{a_1;\theta^2(\omega)}^\dagger  \ldots V_{a_n;\theta^{n+1}(\omega)}^\dagger }{\tr{V_{a_n;\theta^{n+1}(\omega)} \ldots V_{a_1;\theta^2(\omega)} V_{a;\omega} \varrho V_{a;\omega}^\dagger V_{a_1;\theta^2(\omega)}^\dagger  \ldots V_{a_n;\theta^{n+1}(\omega)}^\dagger }}\\
    &= \dfrac{V_{a_n;\theta^{n+1}(\omega)} \ldots V_{a_1;\theta^2(\omega)} \rho' V_{a_1;\theta^2(\omega)}^\dagger  \ldots V_{a_n;\theta^{n+1}(\omega)}^\dagger}{\tr{V_{a_n;\theta^{n+1}(\omega)} \ldots V_{a_1;\theta^2(\omega)} \rho' V_{a_1;\theta^2(\omega)}^\dagger  \ldots V_{a_n;\theta^{n+1}(\omega)}^\dagger }}\\
    &= \rho^{(n)}_{\rho';\theta(\omega)}(a_1\,a_2,\ldots)
\end{align}
Therefore we have that the trajectory started at $\varrho$ with disorder $\omega$ purifies with $\mbQ_{\varrho;\omega}$-probability $1$ whenever $\varrho': = V_{a;\theta(\omega)}\cdot \varrho \in\mbS_D$ but as $\mcV$ is a disordered perfect Kraus measurement we have that for any state $\varrho$,  $\Pr$-almost every $\omega$ must have some $a\in\mcA$ with $V_{a;\theta(\omega)}\cdot \varrho \in \mbS_D$. Therefore we have that 
\begin{equation}
    \Pr\left(X \Delta \theta^{-1}(X) \right)  = \Pr(X\setminus \theta^{-1}(X)) = \Pr(X) - \Pr(X\cap \theta^{-1}(X))= 0 
\end{equation}
where the first equality come from the previous observation that $\theta^{-1}(X)\subseteq X$ $\Pr$-almost surely and last equality comes again from the facts that $\theta^{-1}(X)\subseteq X$ $\Pr$-almost surely and that $\theta$ is measure preserving. 





\iffalse
Now we prove that $X$ is invariant under $\theta$ whence $\Pr(X) \in \{0,1\}$ follows from the ergodicity of $\theta$. To see this let $\omega\in \theta^{-1}(X)\setminus\Xi$. Then, by the original definition of $X$, for any $\varrho'\in\mbS_d$, 
%
\begin{equation}\label{Purification event is 0-1, Eqn 1}
\mbQ_{\varrho'; \theta(\omega)}\left(M_{\varrho; \theta(\omega)}^{(m)} = 1\right) 
     =
1.
\end{equation}
%
Let $\varrho\in\mbS_d$ be arbitrary. For all $a\in\mcA$ with $\mbQ_{\varrho; \omega}(\pi_1^{-1}\{a\})>0$, let $\varrho(a; \omega)$ denote $V_{{a};{\omega}}\cdot\varrho$. By \eqref{Purification event is 0-1, Eqn 1} with $\varrho' = \varrho(a; \omega)$, we have
%
\begin{equation}\label{Purification event is 0-1, Eqn 2}
\mbQ_{\varrho(a; \theta(\omega)); \theta(\omega)}\left(M_{\varrho(a; \theta(\omega)); \theta(\omega)}^{(m)} = 1\right) 
     =
1.
\end{equation}
%
Let now $S:\mcA^\mbN\to\mcA^\mbN$ denote the shift $S(a_1, a_2, \dots) = (a_2, \dots)$. Let $\mbQ_{\varrho;\omega}\left(\cdot\,\vert\,\pi_1^{-1}\{a\}\right)$ denote the conditional probability and $S_*\mbQ_{\varrho;\omega}\left(\cdot\,\vert\,\pi_1^{-1}\{a\}\right)$ denote the pushforward measure. Then
%
\begin{align*}
S_*\mbQ_{\varrho;\omega}\Big(\pi_n^{-1}\{(a_1, \dots, a_n)\}\vert\pi_{1}^{-1}\{a\}\Big)
    &= 
\frac{\mbQ_{\varrho;\omega}\Big(S^{-1}\left(\pi_{n+1}^{-1}\{(a, a_1, \dots, a_n)\}\right)\cap \pi_1^{-1}\{a\}\Big)}{\mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right)}\\
    &= 
\frac{\mbQ_{\varrho;\omega}\left(\pi_{n+1}^{-1}\{(a, a_1, \dots, a_n)\}\right)}{\mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right)}\\
    &=
\frac{\operatorname{tr}\left(
    V_{(a, a_1, \dots, a_n); \omega}^{(n)}\varrho V_{(a, a_1, \dots, a_n); \omega}^{(n)\dagger}
    \right)}{\operatorname{tr}\left(V_{a;\omega}\varrho V_{a;\omega}^\dagger\right)}
                            \\
    &= 
\tr{
V_{(a_1, \dots, a_n); \theta(\omega)}^{(n)}\varrho(a, \theta(\omega))V_{(a_1, \dots, a_n); \theta(\omega)}^{(n)\dagger}
}\\
    &=
\mbQ_{\varrho(a, \theta(\omega));\theta(\omega)}\left(\pi_n^{-1}\{(a_1, \dots, a_n)\}\right)
\end{align*}
%
for any $a_1, \dots, a_n\in\mcA$ and $a\in\mcA$ with $\mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right) > 0$. In particular, 
%
\begin{equation}\label{Purification event is 0-1, Eqn 3}
    S_*\mbQ_{\varrho;\omega}\Big(\cdot\vert\pi_{1}^{-1}\{a\}\Big)
    =
    \mbQ_{\varrho(a; \theta(\omega)); \theta(\omega)}.
\end{equation}
%
Because
%
\[
    \mbQ_{\varrho; \omega}
    \left(  
        M_{\varrho; \omega}^{(m)} = 1
    \right)
    =
    \sum_{a\,:\, \mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right) > 0}
    \mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right)
     S_*\mbQ_{\varrho;\omega}\Big(M_{\varrho(a; \theta(\omega)); \theta(\omega)}^{(m)} = 1\,\big\vert\,\pi_{1}^{-1}\{a\}\Big),
\]
%
from \eqref{Purification event is 0-1, Eqn 1} and \eqref{Purification event is 0-1, Eqn 3} we have 
%
\begin{align*}
     \mbQ_{\varrho; \omega}
    \left(  
        M_{\varrho; \omega}^{(m)} = 1
    \right)
    &=
    \sum_{a\,:\, \mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right) > 0}
    \mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right)
     \mbQ_{\varrho(a; \theta(\omega)); \theta(\omega)}\Big(M_{\varrho(a; \theta(\omega)); \theta(\omega)}^{(m)} = 1\Big)\\
     &= 
     \sum_{a\,:\, \mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right) > 0}
    \mbQ_{\varrho;\omega}\left(\pi_1^{-1}\{a\}\right)\\
    &= 1,
\end{align*}
%
whereby $\omega\in X$. Since $\Xi$ is a null set, this implies that $X$ is essentially $\theta$-invariant. Thus, ergodicity of $\theta$ allows us to conclude $\Pr(X)\in\{0, 1\}$.
\fi
\end{proof}







%Not including this proof here anymore because it is an immediate corollary of Theorem 3. No need to prove the same thing twice. 
\iffalse 
Before we provide the proof of Theorem \ref{Main theorem} we shall state few more relevant results for the proof of Theorem \ref{Main theorem} below. 

Now we proceed to provide a proof of theorem \ref{Main theorem} which we shall restate below: 
\secondresult*
%
\begin{proof}[Proof of Theorem \ref{Main theorem}]
First recall that $\mcV$ purifies if and only if $\Pr(X) = 1$. Therefore one direction of the proof is obtained from Proposition \ref{Main theorem, technical part} as follows: assume $\Pr(X) = 0$ there $\Pr$-almost surely for all $n\in\mbN$ and for all all $\bar{a} = (a_1\ldots a_n)\in\mcA^n$ there is a mixed state $\psi(\omega)$ and some $\lambda^{(n)}_{\bar{a}}\geq0$ such that for all $(a_1\ldots a_n)\in\mcA^n$ we have that  
        \begin{equation}
            V_{a_n;\theta^{n}(\omega)} \ldots V_{a_1;\omega} \psi(\omega)V_{a_1;\omega}^\dagger V_{a_n;\theta^{n}(\omega)}^\dagger \sim \lambda^{(n)}_{\bar{a}} \psi(\omega)
        \end{equation}
    Then from Lemma \ref{Dark subspaces: Lemma 4, Kum & Maas} we have that for $p = \proj(\psi)$, the projection on to support of $\psi$, we must have that 
        \begin{equation}\label{projectionprop}
            pV_{a_1;\theta(\omega)}^\dagger\ldots V_{a_n;\theta^n(\omega)}^\dagger V_{a_n; \theta^n(\omega)}\ldots V_{a_1; \theta(\omega)}p = \lambda^{(n)}_{\bar{a}} p
        \end{equation}
    Since $P$ has rank $\geq 2$, due to $\psi(\omega)$ begin a mixed state we have proved that whenever $\Pr(X) = 0$, then for $\Pr$-almost every $\omega$  there must exists a projection $p$ of rank at least $2$ such that \ref{projectionprop} holds. Thus whenever \dpur holds we must have that $\mcV$ asymptotically purifies.  
    
    For the converse assume that $\Pr$-almost surely there is some projection $p$ of rank at least 2 such that for all $n\in\mbN$ and $\bar{a}=(a_1,\ldots a_n)\in\mcA^n$ there is some $\lambda_{\bar{a}}^{(n)}\geq 0$ such that \eqref{projectionprop} holds $\Pr$-almost surely. Then let $\varrho = p/(\rank{p})$ then $\varrho\in\mbS_D$ and we have that from Lemma \ref{Dark subspaces: Equivalent notion of dark subspaces} it must be the case that for all $n\in\mbN$
        \begin{equation}
            V^{(n)}_{\bar{a};\omega} \varrho V^{(n)}_{\bar{a};\omega } \sim \lambda 
        \end{equation}
    This gives us that 
        \begin{equation}
            \tr{\left(\rho^{(n)}_{\varrho; \omega}(\bar{a})\right)^2} <
        \tr{\rho^{(n)}_{\varrho; \omega}(\bar{a})}
        =
        1
        \end{equation}
    I.E., $\Pr$-almost surely there is some state $\varrho$ such that the trajectory started at $\varrho$ does not asymptotically purifies. Thus we have proved that when \dpur does not hold $\mcV$ does not purify. This concludes the proof of the theorem. 
\end{proof}
\fi 


